On Some Variants of the Gauss Circle Problem

The Gauss Circle Problem concerns finding asymptotics for the number of lattice point lying inside a circle in terms of the radius of the circle. The heuristic that the number of points is very nearly the area of the circle is surprisingly accurate. In this work, we describe two variants of the Gauss Circle problem that exhibit similar characteristics. The first variant concerns sums of Fourier coefficients of $\text{GL}(2)$ cusp forms. These sums behave very similarly to the error term in the Gauss Circle problem. We introduce new Dirichlet series with coefficients that are squares of partial sums of Fourier coefficients of cusp forms. We study the meromorphic properties of these Dirichlet series and use these series to give new perspectives on the mean square of the size of sums of these Fourier coefficients. The second variant concerns the number of lattice points of bounded size on one-sheeted hyperboloids. This problem is very similar to counting the number of lattice points within a spheres of various dimensions, except with the additional constraint of lying on a hyperboloid. It turns out that this problem is equivalent to estimating sums of the shape $\sum r_d(n^2 + h)$, where $r_d(m)$ is the number of representations of $m$ as a sum of $d$ squares. We prove improved smoothed and sharp estimates of the second moment of these sums, yielding improved estimates of the number of lattice points.

==> BjarneThesisTitles.tex <==
% Redefine alphano commands

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
  
  \ChNameVar{\Huge\sc}    % sets the style for name
  \ChNumVar{\Huge\sc}         % sets the style for digit
  \ChTitleVar{\Huge\bf\centering} % sets the style for title
  \ChRuleWidth{4pt}        % Set RW=4pt
  %\ChNameUpperCase         % Make name uppercase
  \ChNameAsIs         % Make name uppercase
  \ChTitleAsIs

  \renewcommand{\DOCH}{%
    %\setlength{\fboxrule}{\RW} % Let fbox lines be controlled by
                               % \ChRuleWidth
    %\fbox{\CNV\FmN{\@chapapp}\space \CNoV\thechapter}\par\nobreak
    \thispagestyle{empty}
    \vskip 80\p@
    \begin{center}
    %\CNV\FmN{\@chapapp}\space \CNoV\thechapter\par\nobreak
    \CNV\FmN{\@chapapp} \TheAlphaChapter\par\nobreak
    \begin{tabular*}{\textwidth}{c}
      \hline
    \end{tabular*}
    %\line(1,0){5in}\\
    \end{center}
    %\vskip 20\p@
    }

  \renewcommand{\DOTI}[1]{%
    \CTV\FmTi{#1}\par\nobreak
    \vskip 40\p@
    {\newpage}
    }
  \renewcommand{\DOTIS}[1]{%
    \CTV\FmTi{#1}\par\nobreak
    \vskip 40\p@
    }
\makeatother



==> Content/vita.tex <==

\begin{center}
David Lowry-Duda \\
b. October 12, 1988 \\
Atlanta, GA, USA
\end{center}


\section*{Education}

\begin{itemize}

  \item Brown University, Providence, RI, 2011--2017

    Ph.D.\ in Mathematics, May 2017

    M.Sc.\ in Mathematics, 2015

  \item Georgia Institute of Technology, Atlanta, GA, 2007--2011

    B.S.\ in Applied Mathematics, 2011, \emph{summa cum laude}

    B.S.\ in International Affairs and Modern Languages, 2011, \emph{summa cum laude}

  \end{itemize}


\section*{Honors and Awards}


\begin{itemize}

  \item 2012--2017, National Science Foundation Graduate Student Fellowship
  \item 2011, NSF MCTP Scholar of Georgia Tech
  \item 2007--2011, Ronald L.\ Martin President's Scholar of Georgia Tech
  \item 2010, Reginald S.\ Fleet Scholar in Budapest, Hungary
  \item 2009, Reginald S.\ Fleet Scholar in Brussels, Belgium
  \item 2008, Reginald S.\ Fleet Scholar in Mexico City, Mexico
  \item 2004, Eagle Scout

\end{itemize}


\section*{Teaching Experience}

\begin{itemize}

  \item Teaching Fellow,
    MATH 0100 Introduction to Calculus II, Brown University, Fall 2016
  \item Instructor \& Course Developer,
    MATH 0420 Elementary Number Theory, Brown University, Spring 2016
  \item Instructor \& Course Developer,
    CEMA 0903 Elementary Number Theory: An Introduction to Higher Mathematics,
    Brown University, Summer 2015
  \item Teaching Fellow,
    MATH 0170 Advanced Placement Calculus II, Brown University, Fall 2014
  \item Instructor \& Course Developer,
    CEMA 0903 Elementary Number Theory: An Introduction to Higher Mathematics,
    Brown University, Summer 2014
  \item Instructor \& Course Developer,
    CEMA 0903 Elementary Number Theory, Brown University, Summer 2014
  \item Teaching Assistant,
    MATH 0100 Introduction to Calculus II, Brown University, Fall 2013
  \item Instructor \& Course Developer,
    CEMA 0903 Elementary Number Theory: An Introduction to Higher Mathematics,
    Brown University, Summer 2013
  \item Teaching Assistant,
    MATH 0090 Introduction to Calculus I, Brown University, Fall 2012
  \item Teaching Assistant,
    MATH 2401 Calculus III, Georgia Tech, Spring 2011
  \item Teaching Assistant,
    MATH 1502 Calculus II, Georgia Tech, Fall 2010
  \item Teaching Assistant,
    MATH 1501 Calculus I, Georgia Tech, Fall 2009
  \item Teaching Assistant,
    MATH 1502 Calculus II, Georgia Tech, Fall 2008

\end{itemize}


\section*{Service and Professional Activities}

\begin{itemize}
  \item Sheridan Center for Teaching and Learning

    \begin{itemize}
      \item  Sheridan Center teaching consultant,  2014 -- present % chktex 8
      \item  Sheridan Center Certificate IV, 2014 -- 2016 % chktex 8
      \item  Sheridan Center Certificate I, 2013 -- 2014 % chktex 8
    \end{itemize}

  \item Brown University Graduate Student Chapter of the American Mathematical Society

    \begin{itemize}
      \item Founder and President of the Brown University Chapter of the American
        Mathematical Society, 2013--2015
      \item	Co-organizer of the Second Annual Conference for Graduate Students, Hosted by
        the Brown University Graduate Student Chapter of the American Mathematical
        Society, Brown University, February 2015
      \item	Co-organizer of the First Annual Conference for Graduate Students, Hosted by
        the Brown University Graduate Student Chapter of the American Mathematical
        Society, Brown University, March 2014
    \end{itemize}

  \item Research Workshop Participation

    \begin{itemize}
      \item Participant Programmer, SageDays 87: p-adics in SAGE and the LMFDB,
        July~17 -- July~22, 2017. % chktex 8
      \item Semester Visitor, MSRI program on Analytic Number Theory,
        January~17 -- May~26, 2017. % chktex 8
      \item Student Participant, Arizona Winter School on Perfectoid Spaces,
        March~11 -- March~15, 2017. % chktex 8
      \item Project Participant, Arizona Winter School on Analytic Methods in Arithmetic
        Geometry, March~12 -- March~16, 2016. % chktex 8
      \item Semester Research Participant, ICERM semester program in Computational Aspects
        of the Langlands Program, September 8 -- December 3, 2015. % chktex 8
      \item Project Participant, Arizona Winter School on Arithmetic and Higher
        Dimensional Varieties, March~14 -- March~18, 2015. % chktex 8
      \item Project Participant, Arizona Winter School on Arithmetic Statistics, March~15
        -- March~19, 2014. % chktex 8
      \item Visiting Researcher, ICERM IdeaLab in Homomorphic Encryption and
        Cryptography, July~15 -- July~19, 2013. % chktex 8
      \item Participant Programmer, SageDays 45: MDS, Combinatorics, and Representation
        Theory, February~11 -- February~15, 2013. % chktex 8
      \item Semester Research Participant, ICERM semester program in Automorphic Forms,
        Combinatorial Representation Theory, and Multiple Dirichlet Series,
        \href{http://icerm.brown.edu/home}{ICERM}, January 28 -- May 3, 2013. % chktex 8
      \item Research Participant, Georgia Tech REU on Deterministic Methods to Find Primes
        under Dr.\ Ernie Croot, summer 2010.
    \end{itemize}

  \item Moderator and Contributor to Math.StackExchange

\end{itemize}


\section*{Publications}


\begin{itemize}

  \item Alina Bucur, Edgar Costa, Chantal David, Jo\~{a}o Guerreiro, David Lowry-Duda,
    \emph{Traces, High powers and One level density for families of curves over finite fields},
    To appear in the Mathematical Proceedings of the Cambridge Philosophical Society. \\
    Preprint: \url{https://arxiv.org/abs/1610.00164}.

  \item Thomas Hulse, Chan Ieong Kuan, David Lowry-Duda, and Alexander Walker,
    \emph{The Second Moment of Sums of Coefficients of Cusp Forms},
    Journal of Number Theory 173 (2017): 304--331. \\
    Preprint: \url{http://arxiv.org/abs/1512.01299}.

  \item Thomas Hulse, Chan Ieong Kuan, David Lowry-Duda, and Alexander Walker,
    \emph{Short-Interval Averages of Sums of Fourier Coefficients of Cusp Forms},
    Journal of Number Theory 173 (2017): 394--415. \\
    Preprint: \url{http://arxiv.org/abs/1512.05502}.

  \item Thomas Hulse, Chan Ieong Kuan, David Lowry-Duda, and Alexander Walker,
    \emph{Sign Changes of Coefficients and Sums of Coefficients of $L$-functions},
    Journal of Number Theory 177 (2017): 112--135. \\
    \url{http://arxiv.org/abs/1606.00067}.

  \item Paul Carter and David Lowry-Duda,
    \emph{On Functions Whose Mean Value Abscissas are Midpoints, with Connections to Harmonic Functions},
    To appear in Amer. Math. Monthly in 2017. \\
    Preprint: \url{http://arxiv.org/abs/1608.02558}.

  \item David Lowry-Duda,
    \emph{Unexpected Conjectures about -5 Modulo Primes}.
    College Math. J. Vol 46, No. 1, January 2015.\\
    DOI:\ 10.4169/college.math.j.46.1.56.

\end{itemize}


\section*{Presentations}

\begin{itemize}

    \item \emph{On Problems Related to the Gauss Circle Problem},
      Dartmouth Number Theory Seminar,
      Dartmouth, NH,
      March 2017.

    \item \emph{Counting Points on One-Sheeted Hyperboloids},
      MSRI Number Theory Seminar,
      Berkeley, CA,
      February 2017.

    \item \emph{Old and New Results on the Gauss Circle Problem},
      Louisiana Tech, LA,
      January 2017.

    \item Lowry-Duda, D.
      On Iterated Partial Sums of Coefficients of Cusp Forms and Related Topics.
      In: 2016 Maine-Quebec Conference,
      Universit\'{e} Laval, Qu\'{e}bec,
      October 8--9, 2016.

    \item \emph{Functions where midpoints are mean value abscissas, and other questions
      concerning the (not so boring) mean value theorem of calculus},
      Graduate Student Seminar,
      Brown University, RI,
      April 2016.

    \item \emph{Progress Update on Trace Functions in Number Theory},
      Arizona Winter School Project Presentations,
      University of Arizona, AZ,
      March 2016.

    \item \emph{Sign Changes of Sums of Fourier Coefficients of Cusp Forms},
      Texas A\&M Number Theory Seminar,
      Texas A\&M, TX,
      May 2015.

    \item \emph{The Mean Value Theorem and Why It's Not Useless},
      Bard College at Simon's Rock,
      Bard College, MA,
      May 2015.

    \item \emph{Explicit Torsion and Brauer-Manin Obstructions},
      Arizona Winter School Project Presentations,
      University of Arizona, AZ,
      March 2015.

    \item \emph{The Mean Value Theorem, the Real Fundamental Theorem of Calculus},
      Brown Math Department Undergrads Group (MATHDUG),
      Brown University, RI,
      October 2014.

    \item \emph{Analogies in Number Theory: How number theory, function field number
      theory, and random matrices connect and inform},
      Graduate Student Seminar,
      Brown University, RI,
      October 2014.

    \item \emph{A New, Simple Proof of the Prime Number Theorem and Dirichlet's Theorem on
      Primes in Arithmetic Progressions},
      Graduate Student Seminar,
      Brown University, RI,
      February 2014.

    \item \emph{Finding `Perfect' Functional Equations},
      Analytic Number Theory Topics Group,
      Brown University, RI,
      November 2013.

    \item \emph{An Introduction to Sieves with a Look Towards Recent Progress on the Twin
      Prime Conjecture},
      Graduate Student Seminar,
      Brown University, RI,
      October 2013.

    \item \emph{A Connection between Quadratic Functions and Modular Forms},
      Graduate Student Seminar,
      Brown University, RI,
      June 2013.

    \item \emph{The Erd\"os Discrepancy Problem and Polymath5},
      Graduate Student Seminar,
      Brown University, RI,
      October 2012.

    \item \emph{Tiontobl: An Introduction to Combinatorial Game Theory},
      Graduate Student Seminar,
      Brown University, RI,
      April 2012.

    \item \emph{Deterministic Methods to Find Primes and Polymath4},
      Graduate Student Seminar,
      Brown University, RI,
      November 2011.

    \item \emph{New Results on Deterministic Methods to Find Primes and Polymath4},
      REU Research Session,
      Georgia Institute of Technology, GA,
      March 2011.

    \item \emph{The Interests of Math},
      Club Math,
      Georgia Institute of Technology, GA,
      February 2010.

    \item \emph{The Math and Music of Calculus: The Musical},
      Club Math,
      Georgia Institute of Technology, GA,
      November 2009.

\end{itemize}

\section*{Professional Associations}

\begin{itemize}
  \item American Mathematical Society
  \item Canadian Mathematical Society
  \item Pi Mu Epsilon
\end{itemize}

% vim: tw=90

